AgEncID: Aggregate Encryption Individual Decryption of Key for FPGA Bitstream IP Cores in Cloud

Cloud computing platforms are progressively adopting Field Programmable Gate Arrays to deploy specialized hardware accelerators for specific computational tasks. However, the security of FPGA-based bitstream for Intellectual Property, IP cores from unauthorized interception in cloud environments remains a prominent concern. Existing methodologies for protection of such bitstreams possess several limitations, such as requiring a large number of keys, tying bitstreams to specific FPGAs, and relying on trusted third parties. This paper proposes Aggregate Encryption and Individual Decryption, a cryptosystem based on key aggregation to enhance the security of FPGA-based bitstream for IP cores and to address the pitfalls of previous related works. In our proposed scheme, IP providers can encrypt their bitstreams with a single key for a set S of FPGA boards, with which the bitstreams can directly be decrypted on any of the FPGA boards in S. Aggregate encryption of the key is performed in a way which ensures that the key can solely be obtained onboard through individual decryption employing the board's private key, thus facilitating secure key provisioning. The proposed cryptosystem is evaluated mainly on Zynq FPGAs. The outcomes demonstrate that our cryptosystem not only outperforms existing techniques with respect to resource, time and energy significantly but also upholds robust security assurances.

==> 0_deprecated.tex <==
\section{Abstract}

\subsection{Version 1}
Cloud computing platforms are increasingly using Field Programmable Gate Arrays (FPGAs) to implement hardware accelerators for specific computation tasks. However, the security of FPGA-based bitstream IP cores against unauthorized interception on the cloud is a major concern. Existing bitstream protection techniques have several drawbacks, such as requiring a large number of keys, tying bitstreams to specific FPGAs, and relying on trusted third parties.This paper proposes a cryptosystem based on key aggregation for ensuring the security of FPGA-based bitstream IP cores which partially addresses the pitfalls of previous works. The proposed scheme facilitates single encryption of an IP bitstream to be executed on a set of FPGA boards using a single key. Aggregate encryption is performed for the key which could only be obtained on-board by individual decryption with the private key of the board. The proposed scheme was evaluated on Zynq FPGAs.  The outcomes demonstrate that our technique not only outperforms existing techniques with respect to time and power significantly but also upholds robust security assurances.

\subsection{Version 2}
Cloud computing platforms have integrated Field Programmable Gate Arrays (FPGAs) for implementing hardware accelerators to perform specific computation tasks. Intellectual properties (IPs) for such accelerators owned by a developer must be protected from theft while being transferred and stored on the cloud. We propose a cryptosystem based on {\textbf{key aggregation}} for ensuring the security of FPGA-based bitstream IP cores against unauthorized interception on the cloud. IP stealing not only reduces profits and market shares but also causes damage to the brand's reputation. Our scheme facilitates composite-key encryption where aggregate encryption is performed for an IP to be executed on a set of FPGA boards but individual decryption at each FPGA with a unique decryption key. Experimentation is performed with ZynQ FPGAs. We achieved a reduction of~25\% for both time and power compared to the naive single encryption single decryption (SESD) mechanism. Moreover, our technique requires minimal resource overhead.


\subsection{Version 3}
Cloud computing platforms have integrated Field Programmable Gate Arrays (FPGAs) for implementing hardware accelerators to perform specific computation tasks.  Intellectual properties (IPs) for such accelerators owned by a developer must be protected from theft while being stored and transferred on the cloud. We propose a cryptosystem based on {\textbf{key aggregation}} for ensuring security of FPGA-based bitstream IP cores against unauthorized interception on cloud. IP stealing not only reduce the profits and market shares, but also cause damage to the brand reputation. Our scheme facilitates a composite-key encryption where a single encryption is performed for an IP to be executed on a set of FPGA boards but unique decryption at each FPGA having individual decryption key. Experimentation is performed with ZynQ FPGAs. We achieved a reduction of 25\% for both time and power compared to naive single encryption single decryption (SESD) mechanism. Moreover, our technique requires minimal resource overhead.


% Moreover, with the increase in number of boards of the system, our framework performs better than OEOD with respect to both time and power, as evident from the graphical analysis presented in this paper.


% We achieved a reduction of around 25\% for both time and power compared to one encryption one decryption (OEOD) mechanism, which is adopted in most of the existing works. Moreover, with the increase in number of boards of the system, our framework performs better than OEOD with respect to both time and power, as evident from the graphical analysis presented in this paper. 


% Commercial cloud computing platforms such as Amazon Web Services (AWS), Huawei cloud, Alibaba cloud, have integrated Field Programmable Gate Arrays (FPGAs) for implementing hardware accelerators to perform specific computation tasks. The 
% Intellectual properties (IPs) for such accelerators developed and owned by a developer should be protected from theft while stored and transferred on the cloud. Thus we design a cryptosystem based on {\textbf{key aggregation}} technique for ensuring security of the FPGA-based bitstream IP cores against unauthorized interception on cloud like man-in-middle, eavesdropping, cloning and reverse engineering of bitstream which not only reduces the profits and market share, but also causes the damage to the brand reputation. Our scheme facilitate an ease composite-key encryption where a single encryption is performed for an IP to be executed on a set of FPGAs but unique decryption is done at the FPGAs having individual decryption key. Experimentation is performed with ZynQ FPGAs. We achieved a reduction of around 25\% for both time and power compared to one encryption one decryption (OEOD) mechanism, which is adopted in most of the existing works. Moreover, with the increase in number of boards of the system, our framework performs better than OEOD with respect to both time and power, as evident from the graphical analysis presented in this paper. 


% However, with the increase in number of users, managing real time tasks and ensuring their completion before deadline, pose challenges. Thus system designers have adhered to distributed cloud platforms, where several cloudlets are placed closer to users in order to facilitate quick task execution. Further, reconfigurable hardware  such as FPGAs are deployed by cloud service providers to facilitate hardware acceleration.  These FPGAs  need to be configured with bitstreams that are generally stored in a resource pool of the main cloud and sent to the hardware on demand. 


% Adversaries may intercept such bitstreams to either modify or duplicate and use in other platforms. Hence, cryptographic mechanisms to secure the bitstreams are of utmost importance. In existing works, performing encryption at the main cloud and decryption on the FPGA for each application bitstream incurs high overhead in resource, time and power, and also requires efficient key management. We propose a reverse key aggregate cryptosystem (ReKAC) where a single encryption is performed at the main cloud, yet unique decryption at the FPGA can be done. We thereby obtain a secure transmission mechanism in distributed cloud platform with low time and power. Complexity in key management at the main cloud is also reduced as an aggregate encryption is performed. Experimentation is performed with ZynQ FPGAs. A reduction of around 25\% is obtained for both time and power when ReKAC is used than single encryption single decryption (SESD) mechanism, which is adopted in most of the existing works. Moreover, with the increase in number of boards of the system, ReKAC performs better than SESD with respect to both time and power, as evident from the graphical analysis presented in this paper. 
% %reduction in ReKAC depict that our proposed ReKAC mechanism incurs lower time and energy than that for earlier methods.
% % including generation of multiple keys.


% % , storing and transmission of those and eventually selection of an appropriate one from those keys.



\noindent \textbf{Execution Time.} 
Figures \ref{fig:aes-energy-time} (a) and (b) illustrate  consistent execution time needed by \emph{AgEID} for AES key generation and bitstream encryption respectively in \textit{Experiment 1}, compared to the slower \emph{IEID} approach. \autoref{fig:aes-energy-time} (c) further highlights the significant $5X$ time difference between IEID and AgEID in \textit{Experiment 2}, which poses a considerable cost in handling large bitstreams. These results are obtained from Vivado. In \textit{Experiment 3} \emph{AgEID} perform similar to \emph{IEID} for bitstream encryption if $n = m$. However, key generation is performed at constant time by \emph{AgEID} unlike \emph{IEID} where the time increases with increase in number of boards. For both Scenarios 1 and 2, \emph{AgEID} maintains a constant time requirement in \textit{Experiment 4}, unlike naive mechanisms that requires individual key encryption for each board. \autoref{fig:ageid-energy-time} (a) shows the timing results for \textit{Experiment 4}. This result indicates the CPU time required to execute the $AgEID$'s key encryption algorithm. We observe that the time required for key encryption is comparatively lower than the time required for bitstream encryption.

==> 7_proof.tex <==
\section{Proof of Correctness for $AgEncID$}

The following properties of bilinear pairing~\cite{pairingecc} are used for the proof of basic \emph{AgEncID} scheme where the symbols used below have been defined in Section~\ref{sec:framework}-A:

\begin{itemize}
    \item[] \textit{Property I:} $\hat{e}(a + b, c)=\hat{e}(a, c) \cdot \hat{e}(b, c)$

    \item[] \textit{Property II:} $\hat{e}(a - b, c)= \frac{\hat{e}(a, c)}{\hat{e}(b, c)}$
    \item[] \textit{Property III:} $\hat{e}(a, tb) = \hat{e}(ta, b)$
    \item[] \textit{Property IV:} $\hat{e}(a_1, b_n)=\hat{e}(a, b_{n+1})$
\end{itemize}

\noindent
%Now we are showing the correctness of our proposed encryption-decryption approach.
Next, let  $\hat{m}$  be the decrypted message of an original message $m$.
According to our approach:

\begin{align}
    \hat{m} &= c_3 \cdot \frac{\hat{e}((d_i + \sum\limits_{(j \in S \wedge j \neq i)}g_{n+1-j+i}),c_1)}{\hat{e}(g_{i}, c_{2})} \nonumber\\ 
    &=c_3 \cdot \frac{\hat{e}(({\gamma}g_{i} + \sum\limits_{j \in S} g_{n+1-j+i} - g_{n+1}),\ tg)}{\hat{e}(g_{i}, t(pk + \sum\limits_{j \in S} g _ {n+1-j}))} \nonumber\\
    &=c_3 \cdot \frac{\hat{e}( {\gamma}g_{i} , tg) \hat{e}(\sum\limits_{j \in S}\ g_{n+1-j+i} - g_{n+1}, tg)}{\hat{e}( g_{i}, t{\gamma}g) \hat{e}(g_i, t\sum\limits_{j \in S} g _ {n+1-j})} \tag{using Property I} \nonumber\\
    &=c_3 \cdot \frac{\hat{e}(\sum\limits_{j \in S} g_{n+1-j+i}, tg)}{\hat{e}(tg, \sum\limits_{j \in S}\ g _ {n+1-j+i}) \hat{e}( g_{n+1}, tg)} \tag{using Property II, III} \nonumber\\
    &=c_3 \cdot \frac{1}{\hat{e}(g_{n+1},tg)} \tag{using Property III} \nonumber\\
    &=m \cdot \frac{\hat{e}(g_{n},tg_1)}{\hat{e}(g_{n+1},tg)}  \tag{using Property II}\nonumber\\
    &=m \cdot \frac{\hat{e}(g_{n},tg_1)}{\hat{e}(g_{n},tg_1)}\tag{using Property IV} \nonumber\\
    &=m \tag{$\blacksquare$}
\end{align}
This establishes the correctness of the encryption and decryption algorithms of $AgEncID$.

==> figures/scenario_2.tex <==
\begin{figure*}[h!]
\centering

\subfloat[Encryption]{
    \begin{tikzpicture}[scale=0.3] %use this to change scaling of image
    \begin{axis}%[legend pos=outer north east]
    [    %xmode=log,
      %      log ticks with fixed point,
height=0.8\columnwidth,
width=1\columnwidth,
%xlabel= Accuracy,
%ylabel= Accuracy,
every major tick/.append style={very thick, major tick length=10pt, black},
axis line style = very thick,
tick label style={font=\huge},
xtick = {0,2,4,6,8,10,12},
xticklabels = {0,2,4,6,8,10,12},
ytick = {0,5,10,20,30},
yticklabels = {0,5,10,20,30},
label style={font=\huge},
xlabel=\textbf{Number of Boards},ylabel=\textbf{Execution Time (s)},
grid style = dashed,
grid=both,
legend style=
{at={(0.5, 0.9)}, %use this to change position of legend
anchor=north east,
%legend columns=-1, %use this to change legend style to horizontal
} ,
]


\addplot[color=black, solid, mark=FPGA, line width=2] plot coordinates {

(2, 1.19) 
(4, 5.2) 
(6, 5.2) 
(8, 8.44)
(10, 8.44)
};


\addplot[color=blue, solid, mark=FPGA, line width=2] plot coordinates {

(2, 2.38) 
(4, 7.56) 
(6, 15.58) 
(8, 22.06)
(10, 28.56)
};



\legend{\huge{\bf{AgEID}}\\\huge{\bf{IEID}}\\}
\end{axis}
\end{tikzpicture}
}
\subfloat[Encryption]{
    \begin{tikzpicture}[scale=0.3] %use this to change scaling of image
    \begin{axis}%[legend pos=outer north east]
    [    %xmode=log,
      %      log ticks with fixed point,
height=0.8\columnwidth,
width=1\columnwidth,
%xlabel= Accuracy,
%ylabel= Accuracy,
every major tick/.append style={very thick, major tick length=10pt, black},
axis line style = very thick,
tick label style={font=\huge},
xtick = {0,2,4,6,8,10,12},
xticklabels = {0,2,4,6,8,10,12},
ytick = {0,5,10, 15, 20},
yticklabels = {0,5,10, 15, 20},
label style={font=\huge},
xlabel=\textbf{Number of Boards},ylabel=\textbf{Energy Consumption (J)},
grid style = dashed,
grid=both,
legend style=
{at={(0.5, 0.9)}, %use this to change position of legend
anchor=north east,
%legend columns=-1, %use this to change legend style to horizontal
} ,
]


\addplot[color=black, solid, mark=FPGA, line width=2] plot coordinates {

(2, 2.185) 
(4, 3.932) 
(6, 3.932) 
(8, 5.582)
(10, 5.582)
};


\addplot[color=blue, solid, mark=FPGA, line width=2] plot coordinates {

(2, 4.37) 
(4, 8.302) 
(6, 12.796) 
(8, 16.096)
(10, 18.396)
};

\legend{\huge{\bf{AgEID}}\\\huge{\bf{IEID}}\\}
\end{axis}
\end{tikzpicture}
}

 \caption{Comparison of energy consumption by $AgEID$ vs. $IEID$ for AES bitstream encryption in Scenario 1}
 \label{fig:ageid-energy}
 \vspace{-0.75cm}
\end{figure*}
